10.4m GTC observations of the nearby VHE-detected GRB 190829A/SN 2019oyw

Aims. GRB 190829A (z = 0.0785), detected by Fermi and Swift with two emission episodes separated by a quiescent gap of ~40 s, was also observed by the H.E.S.S. telescopes at Very-High Energy (VHE). We present the 10.4m GTC observations of the afterglow of GRB 190829A and underlying supernova and compare it against a similar GRB 180728A and discuss the implications on underlying physical mechanisms producing these two GRBs. Methods. We present multi-band photometric data along with spectroscopic follow-up observations taken with the 10.4m GTC telescope. Together with the data from the prompt emission, the 10.4m GTC data are used to understand the emission mechanisms and possible progenitor. Results. A detailed analysis of multi-band data of the afterglow demands cooling frequency to pass between the optical and X-ray bands at early epochs and dominant with underlying SN 2019oyw later on. Conclusions. Prompt emission temporal properties of GRB 190829A and GRB 180728A are similar, however the two pulses seem different in the spectral domain. We found that the supernova (SN) 2019oyw associated with GRB 190829A, powered by Ni decay, is of Type Ic-BL and that the spectroscopic/photometric properties of this SN is consistent with those observed for SN 1998bw but evolved comparatively early.

==> bib.tex <==
@ARTICLE{Cano2013,
       author = {{Cano}, Zach},
        title = "{A new method for estimating the bolometric properties of Ibc supernovae}",
      journal = {\mnras},
     keywords = {methods: analytical, methods: statistical, gamma-ray burst: general, super-novae: general, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2013,
        month = sep,
       volume = {434},
       number = {2},
        pages = {1098-1116},
          doi = {10.1093/mnras/stt1048},
archivePrefix = {arXiv},
       eprint = {1306.1488},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013MNRAS.434.1098C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{Wheeler2015,
       author = {{Wheeler}, J. Craig and {Johnson}, V. and {Clocchiatti}, A.},
        title = "{Analysis of late-time light curves of Type IIb, Ib and Ic supernovae}",
      journal = {\mnras},
     keywords = {opacity, radiative transfer, supernovae: general, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2015,
        month = jun,
       volume = {450},
       number = {2},
        pages = {1295-1307},
          doi = {10.1093/mnras/stv650},
archivePrefix = {arXiv},
       eprint = {1411.5975},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015MNRAS.450.1295W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Bufano2012,
       author = {{Bufano}, Filomena and {Pian}, Elena and {Sollerman}, Jesper and
         {Benetti}, Stefano and {Pignata}, Giuliano and {Valenti}, Stefano and
         {Covino}, Stefano and {D'Avanzo}, Paolo and {Malesani}, Daniele and
         {Cappellaro}, Enrico and {Della Valle}, Massimo and {Fynbo}, Johan and
         {Hjorth}, Jens and {Mazzali}, Paolo A. and {Reichart}, Daniel E. and
         {Starling}, Rhaana L.~C. and {Turatto}, Massimo and
         {Vergani}, Susanna D. and {Wiersema}, Klass and {Amati}, Lorenzo and
         {Bersier}, David and {Campana}, Sergio and {Cano}, Zach and
         {Castro-Tirado}, Alberto J. and {Chincarini}, Guido and
         {D'Elia}, Valerio and {de Ugarte Postigo}, Antonio and {Deng}, Jinsong and
         {Ferrero}, Patrizia and {Filippenko}, Alexei V. and {Goldoni}, Paolo and
         {Gorosabel}, Javier and {Greiner}, Jochen and {Hammer}, Francois and
         {Jakobsson}, Pall and {Kaper}, Lex and {Kawabata}, Koji S. and
         {Klose}, Sylvio and {Levan}, Andrew J. and {Maeda}, Keiichi and
         {Masetti}, Nicola and {Milvang-Jensen}, Bo and {Mirabel}, Felix I. and
         {M{\o}ller}, Palle and {Nomoto}, Ken'ichi and {Palazzi}, Eliana and
         {Piranomonte}, Silvia and {Salvaterra}, Ruben and {Stratta}, Giulia and
         {Tagliaferri}, Gianpiero and {Tanaka}, Masaomi and {Tanvir}, Nial R. and
         {Wijers}, Ralph A.~M.~J.},
        title = "{The Highly Energetic Expansion of SN 2010bh Associated with GRB 100316D}",
      journal = {\apj},
     keywords = {supernovae: general, supernovae: individual: SN 2010bh GRB 100316D, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2012,
        month = jul,
       volume = {753},
       number = {1},
          eid = {67},
        pages = {67},
          doi = {10.1088/0004-637X/753/1/67},
archivePrefix = {arXiv},
       eprint = {1111.4527},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012ApJ...753...67B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{Pian2006,
       author = {{Pian}, E. and {Mazzali}, P.~A. and {Masetti}, N. and {Ferrero}, P. and
         {Klose}, S. and {Palazzi}, E. and {Ramirez-Ruiz}, E. and
         {Woosley}, S.~E. and {Kouveliotou}, C. and {Deng}, J. and
         {Filippenko}, A.~V. and {Foley}, R.~J. and {Fynbo}, J.~P.~U. and
         {Kann}, D.~A. and {Li}, W. and {Hjorth}, J. and {Nomoto}, K. and
         {Patat}, F. and {Sauer}, D.~N. and {Sollerman}, J. and
         {Vreeswijk}, P.~M. and {Guenther}, E.~W. and {Levan}, A. and
         {O'Brien}, P. and {Tanvir}, N.~R. and {Wijers}, R.~A.~M.~J. and
         {Dumas}, C. and {Hainaut}, O. and {Wong}, D.~S. and {Baade}, D. and
         {Wang}, L. and {Amati}, L. and {Cappellaro}, E. and
         {Castro-Tirado}, A.~J. and {Ellison}, S. and {Frontera}, F. and
         {Fruchter}, A.~S. and {Greiner}, J. and {Kawabata}, K. and
         {Ledoux}, C. and {Maeda}, K. and {M{\o}ller}, P. and {Nicastro}, L. and
         {Rol}, E. and {Starling}, R.},
        title = "{An optical supernova associated with the X-ray flash XRF 060218}",
      journal = {\nat},
     keywords = {Astrophysics},
         year = 2006,
        month = aug,
       volume = {442},
       number = {7106},
        pages = {1011-1013},
          doi = {10.1038/nature05082},
archivePrefix = {arXiv},
       eprint = {astro-ph/0603530},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006Natur.442.1011P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{Patat2001,
       author = {{Patat}, Ferdinando and {Cappellaro}, Enrico and {Danziger}, John and
         {Mazzali}, Paolo A. and {Sollerman}, Jesper and {Augusteijn}, Thomas and
         {Brewer}, James and {Doublier}, Vanessa and
         {Gonzalez}, Jean Fran{\c{c}}ois and {Hainaut}, Olivier and
         {Lidman}, Chris and {Leibundgut}, Bruno and {Nomoto}, Ken'ichi and
         {Nakamura}, Takayoshi and {Spyromilio}, Jason and {Rizzi}, Luca and
         {Turatto}, Massimo and {Walsh}, Jeremy and {Galama}, Titus J. and
         {van Paradijs}, Jan and {Kouveliotou}, Chryssa and
         {Vreeswijk}, Paul M. and {Frontera}, Filippo and {Masetti}, Nicola and
         {Palazzi}, Eliana and {Pian}, Elena},
        title = "{The Metamorphosis of SN 1998bw}",
      journal = {\apj},
     keywords = {Gamma Rays: Bursts, Stars: Supernovae: General, supernovae: individual (SN 1998bw), Astrophysics},
         year = 2001,
        month = jul,
       volume = {555},
       number = {2},
        pages = {900-917},
          doi = {10.1086/321526},
archivePrefix = {arXiv},
       eprint = {astro-ph/0103111},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2001ApJ...555..900P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Schlafly2011,
       author = {{Schlafly}, Edward F. and {Finkbeiner}, Douglas P.},
        title = "{Measuring Reddening with Sloan Digital Sky Survey Stellar Spectra and Recalibrating SFD}",
      journal = {\apj},
     keywords = {dust, extinction, Galaxy: stellar content, ISM: clouds, Astrophysics - Galaxy Astrophysics},
         year = 2011,
        month = aug,
       volume = {737},
       number = {2},
          eid = {103},
        pages = {103},
          doi = {10.1088/0004-637X/737/2/103},
archivePrefix = {arXiv},
       eprint = {1012.4804},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011ApJ...737..103S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{2020ApJ...893..148R,
       author = {{Rueda}, J.~A. and {Ruffini}, Remo and {Karlica}, Mile and
         {Moradi}, Rahim and {Wang}, Yu},
        title = "{Magnetic Fields and Afterglows of BdHNe: Inferences from GRB 130427A, GRB 160509A, GRB 160625B, GRB 180728A, and GRB 190114C}",
      journal = {\apj},
     keywords = {Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Cosmology and Nongalactic Astrophysics, General Relativity and Quantum Cosmology},
         year = 2020,
        month = apr,
       volume = {893},
       number = {2},
          eid = {148},
        pages = {148},
          doi = {10.3847/1538-4357/ab80b9},
archivePrefix = {arXiv},
       eprint = {1905.11339},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020ApJ...893..148R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2019ApJ...874...39W,
       author = {{Wang}, Y. and {Rueda}, J.~A. and {Ruffini}, R. and {Becerra}, L. and
         {Bianco}, C. and {Becerra}, L. and {Li}, L. and {Karlica}, M.},
        title = "{Two Predictions of Supernova: GRB 130427A/SN 2013cq and GRB 180728A/SN 2018fip}",
      journal = {\apj},
     keywords = {binaries: general, black hole physics, gamma-ray burst: general, hydrodynamics, stars: neutron, supernovae: general, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2019,
        month = mar,
       volume = {874},
       number = {1},
          eid = {39},
        pages = {39},
          doi = {10.3847/1538-4357/ab04f8},
archivePrefix = {arXiv},
       eprint = {1811.05433},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019ApJ...874...39W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2018ATel11898....1H,
       author = {{Heintz}, K.~E. and {Izzo}, L. and {Rossi}, A. and
         {de Ugarte Postigo}, A. and {Malesani}, D.~B. and {Perley}, D.~A. and
         {Thoene}, C.~C. and {Fynbo}, J.~P.~U. and {Milvang-Jensen}, B. and
         {Kann}, D.~A. and {Tanvir}, N.~R. and {Levan}, A.~J. and {Schulze}, S. and
         {Pugliese}, G.},
        title = "{GRB 180728A: No evidence of SN in early VLT/X-shooter spectra}",
      journal = {The Astronomer's Telegram},
     keywords = {Gamma-Ray Burst, Supernovae},
         year = 2018,
        month = jul,
       volume = {11898},
        pages = {1},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018ATel11898....1H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2018GCN.23181....1S,
       author = {{Selsing}, J. and {Izzo}, L. and {Rossi}, A. and {Malesani}, D.~B. and
         {Heintz}, K.~E. and {Schady}, P. and {Starling}, R.~L.~C. and
         {Sollerman}, J. and {Leloudas}, G. and {Cano}, Z. and
         {Fynbo}, J.~P.~U. and {Valle}, M.~D. and {Pian}, E. and {Kann}, D.~A. and
         {Perley}, D.~A. and {Palazzi}, E. and {Klose}, S. and {Hjorth}, J. and
         {Covino}, S. and {D'Elia}, V. and {Tanvir}, N.~R. and {Levan}, A.~J. and
         {Hartmann}, D. and {Kouveliotou}, C.},
        title = "{GRB 180728A: classification of the associated SN 2018fip.}",
      journal = {GRB Coordinates Network},
         year = 2018,
        month = jan,
       volume = {23181},
        pages = {1},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018GCN.23181....1S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2018GCN.23143....1L,
       author = {{Lipunov}, V. and {Gorbovskoy}, E. and {Tiurina}, N. and {Vlasenko}, D. and
         {Kornilov}, V. and {Kuznetsov}, A. and {Chazov}, V. and {Gorbunov}, I. and
         {Zimnukhov}, D. and {Kuvshinov}, D. and {Balanutsa}, P. and
         {Vladimirov}, V. and {Buckley}, D. and {Rebolo}, R. and {Serra}, M. and
         {Lodieu}, N. and {Israelian}, G. and {Suarez-Andres}, L. and
         {Tlatov}, A. and {Senik}, V. and {Dormidontov}, D. and {Podesta}, R. and
         {Podesta}, F. and {Lopez}, C. and {Francile}, C. and {Levato}, H. and
         {Gres}, O. and {Budnev}, N.~M. and {Ishmuhametova}, Y. and
         {Gabovich}, A. and {Yurkov}, V. and {Sergienko}, Y.},
        title = "{GRB 180728A: MASTER early polarization and 19 days monitoring.}",
      journal = {GRB Coordinates Network},
         year = 2018,
        month = jan,
       volume = {23143},
        pages = {1},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018GCN.23143....1L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2018GCN.23142....1I,
       author = {{Izzo}, L. and {Rossi}, A. and {Malesani}, D.~B. and {Heintz}, K.~E. and
         {Selsing}, J. and {Schady}, P. and {Starling}, R.~L.~C. and
         {Sollerman}, J. and {Leloudas}, G. and {Cano}, Z. and
         {Fynbo}, J.~P.~U. and {Valle}, M.~D. and {Pian}, E. and {Kann}, D.~A. and
         {Perley}, D.~A. and {Palazzi}, E. and {Klose}, S. and {Hjorth}, J. and
         {Covino}, S. and {D'Elia}, V. and {Tanvir}, N.~R. and {Levan}, A.~J. and
         {Hartmann}, D. and {Kouveliotou}, C.},
        title = "{GRB 180728A: discovery of the associated supernova.}",
      journal = {GRB Coordinates Network},
         year = 2018,
        month = jan,
       volume = {23142},
        pages = {1},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018GCN.23142....1I},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2018GCN.23102....1S,
       author = {{Sharma}, V. and {Bhattacharya}, D. and {Bhalerao}, V. and {Rao}, A.~R. and
         {Vadawale}, S.},
        title = "{GRB 180728A: AstroSat CZTI detection.}",
      journal = {GRB Coordinates Network},
         year = 2018,
        month = jan,
       volume = {23102},
        pages = {1},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018GCN.23102....1S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2018GCN.23067....1H,
       author = {{Heintz}, K.~E. and {Izzo}, L. and {Rossi}, A. and
         {de Ugarte Postigo}, A. and {Malesani}, D.~B. and {Perley}, D.~A. and
         {Thoene}, C.~C. and {Fynbo}, J.~P.~U. and {Milvang-Jensen}, B. and
         {Kann}, D.~A. and {Tanvir}, N.~R. and {Levan}, A.~J. and {Schulze}, S. and
         {Pugliese}, G. and {Weak}, N.},
        title = "{GRB 180728A: No evidence of SN in early VLT/X-shooter spectra.}",
      journal = {GRB Coordinates Network},
         year = 2018,
        month = jan,
       volume = {23067},
        pages = {1},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018GCN.23067....1H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2018GCN.23066....1R,
       author = {{Ruffini}, R. and {Aimuratov}, Y. and {Bianco}, C.~L. and {Chen}, Y.~C. and
         {Fuksman}, D.~M. and {Karlica}, M. and {Moradi}, R. and {Primorac}, D. and
         {Rueda}, J.~A. and {Sahakyan}, N. and {Wang}, Y.},
        title = "{GRB 180728A: A long GRB of the X-ray flash (XRF) subclass, expecti=.}",
      journal = {GRB Coordinates Network},
         year = 2018,
        month = jan,
       volume = {23066},
        pages = {1},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018GCN.23066....1R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2018GCN.23064....1L,
       author = {{Laporte}, S.~J. and {Starling}, R.~L.~C.},
        title = "{GRB 180728A: Swift/UVOT Detection.}",
      journal = {GRB Coordinates Network},
         year = 2018,
        month = jan,
       volume = {23064},
        pages = {1},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018GCN.23064....1L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2018GCN.23061....1F,
       author = {{Frederiks}, D. and {Golenetskii}, S. and {Aptekar}, R. and
         {Kozlova}, A. and {Lysenko}, A. and {Svinkin}, D. and {Tsvetkova}, A. and
         {Ulanov}, M. and {Cline}, T.},
        title = "{Konus-Wind observation of the bright nearby GRB 180728A.}",
      journal = {GRB Coordinates Network},
         year = 2018,
        month = jan,
       volume = {23061},
        pages = {1},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018GCN.23061....1F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2018GCN.23055....1R,
       author = {{Rossi}, A. and {Izzo}, L. and {Milvang-Jensen}, B. and {Perley}, D.~A. and
         {de Ugarte Postigo}, A. and {Kann}, D.~A. and {Levan}, A.~J. and
         {Tanvir}, N.~R. and {Covino}, S. and {Malesani}, D.~B.},
        title = "{GRB 180728A: VLT/X-shooter redshift of a nearby energetic GRB.}",
      journal = {GRB Coordinates Network},
         year = 2018,
        month = jan,
       volume = {23055},
        pages = {1},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018GCN.23055....1R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2018GCN.23054....1M,
       author = {{Markwardt}, C.~B. and {Barthelmy}, S.~D. and {Cummings}, J.~R. and
         {Krimm}, H.~A. and {Lien}, A.~Y. and {Palmer}, D.~M. and
         {Sakamoto}, T. and {Stamatikos}, M. and {Starling}, R.~L.~C. and
         {Ukwatta}, T.~N.},
        title = "{GRB 180728A: Swift-BAT refined analysis.}",
      journal = {GRB Coordinates Network},
         year = 2018,
        month = jan,
       volume = {23054},
        pages = {1},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018GCN.23054....1M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2018GCN.23052....1T,
       author = {{Tohuvavohu}, A. and {Laporte}, S.~J. and {Kennea}, J.~A. and
         {Osborne}, J.~P. and {Page}, K.~L. and {Beardmore}, A.~P. and
         {D'Ai}, A. and {Melandri}, A. and {D'Avanzo}, P. and
         {Starling}, R.~L.~C.},
        title = "{GRB 180728A: Swift-XRT refined Analysis.}",
      journal = {GRB Coordinates Network},
         year = 2018,
        month = jan,
       volume = {23052},
        pages = {1},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018GCN.23052....1T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2018GCN.23051....1O,
       author = {{Osborne}, J.~P. and {Beardmore}, A.~P. and {Evans}, P.~A. and
         {Goad}, M.~R.},
        title = "{GRB 180728A: Enhanced Swift-XRT position.}",
      journal = {GRB Coordinates Network},
         year = 2018,
        month = jan,
       volume = {23051},
        pages = {1},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018GCN.23051....1O},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2018GCN.23050....1L,
       author = {{Lipunov}, V. and {Gorbovskoy}, E. and {Tiurina}, N. and {Vlasenko}, D. and
         {Kornilov}, V. and {Kuznetsov}, A. and {Chazov}, V. and {Gorbunov}, I. and
         {Zimnukhov}, D. and {Kuvshinov}, D. and {Balanutsa}, P. and
         {Vladimirov}, V. and {Buckley}, D. and {Rebolo}, R. and {Serra}, M. and
         {Lodieu}, N. and {Israelian}, G. and {Suarez-Andres}, L. and
         {Tlatov}, A. and {Senik}, V. and {Dormidontov}, D. and {Podesta}, R. and
         {Podesta}, F. and {Lopez}, C. and {Francile}, C. and {Levato}, H. and
         {Gres}, O. and {Budnev}, N.~M. and {Ishmuhametova}, Y. and
         {Gabovich}, A. and {Yurkov}, V. and {Sergienko}, Y.},
        title = "{GRB 180728A: MASTER OT J165415.75-540239.27 is the Optical Counterpart of GRB.}",
      journal = {GRB Coordinates Network},
         year = 2018,
        month = jan,
       volume = {23050},
        pages = {1},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018GCN.23050....1L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2018GCN.23049....1P,
       author = {{Perri}, M. and {Evans}, P.~A. and {Osborne}, J.~P. and
         {Burrows}, D.~N. and {Kennea}, J.~A. and {Cusumano}, G.},
        title = "{GRB 180728A: Swift-XRT observations.}",
      journal = {GRB Coordinates Network},
         year = 2018,
        month = jan,
       volume = {23049},
        pages = {1},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018GCN.23049....1P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2018GCN.23048....1L,
       author = {{Lipunov}, V. and {Gorbovskoy}, E. and {Tiurina}, N. and {Vlasenko}, D. and
         {Kornilov}, V. and {Kuznetsov}, A. and {Chazov}, V. and {Gorbunov}, I. and
         {Zimnukhov}, D. and {Kuvshinov}, D. and {Balanutsa}, P. and
         {Vladimirov}, V. and {Buckley}, D. and {Rebolo}, R. and {Serra}, M. and
         {Lodieu}, N. and {Israelian}, G. and {Suarez-Andres}, L. and
         {Tlatov}, A. and {Senik}, V. and {Dormidontov}, D. and {Podesta}, R. and
         {Podesta}, F. and {Lopez}, C. and {Francile}, C. and {Levato}, H. and
         {Gres}, O. and {Budnev}, N.~M. and {Ishmuhametova}, Y. and
         {Gabovich}, A. and {Yurkov}, V. and {Sergienko}, Y.},
        title = "{GRB 180728A: MASTER OT (= new object) detection.}",
      journal = {GRB Coordinates Network},
         year = 2018,
        month = jan,
       volume = {23048},
        pages = {1},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018GCN.23048....1L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2018GCN.23046....1S,
       author = {{Starling}, R.~L.~C. and {Barthelmy}, S.~D. and {Lien}, A.~Y. and
         {Moss}, M.~J. and {Page}, K.~L. and {Palmer}, D.~M.},
        title = "{GRB 180728A: Swift detection of a bright burst.}",
      journal = {GRB Coordinates Network},
         year = 2018,
        month = jan,
       volume = {23046},
        pages = {1},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018GCN.23046....1S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2020MNRAS.tmp.1856R,
       author = {{Rhodes}, L. and {van der Horst}, A.~J. and {Fender}, R. and
         {Monageng}, I.~M. and {Anderson}, G.~E. and {Antoniadis}, J. and
         {Bietenholz}, M.~F. and {B{\"o}ttcher}, M. and {Bright}, J.~S. and
         {Green}, D.~A. and {Kouveliotou}, C. and {Kramer}, M. and
         {Motta}, S.~E. and {Wijers}, R.~A.~M.~J. and {Williams}, D.~R.~A. and
         {Woudt}, P.~A.},
        title = "{Radio Afterglows of Very High Energy Gamma-Ray Bursts 190829A and 180720B}",
      journal = {\mnras},
     keywords = {GRB 180720B, gamma-ray bursts: individual: GRB 190829A, radio continuum: transients, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2020,
        month = jun,
          doi = {10.1093/mnras/staa1715},
archivePrefix = {arXiv},
       eprint = {2004.01538},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020MNRAS.tmp.1856R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2020arXiv200311252F,
       author = {{Fraija}, N. and {Veres}, P. and {Beniamini}, P. and {Galvan-Gamez}, A. and
         {Metzger}, B.~D. and {Barniol Duran}, R. and {Becerra}, R.~L.},
        title = "{On the origin of the multi-GeV photons from the closest burst with intermediate luminosity: GRB 190829A}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - High Energy Astrophysical Phenomena},
         year = 2020,
        month = mar,
          eid = {arXiv:2003.11252},
        pages = {arXiv:2003.11252},
archivePrefix = {arXiv},
       eprint = {2003.11252},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020arXiv200311252F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2020arXiv200100648C,
       author = {{Chand}, Vikas and {Banerjee}, Ankush and {Gupta}, Rahul and {Dimple} and
         {Pal}, Partha Sarathi and {Joshi}, Jagdish C. and {Zhang}, Bin-Bin and
         {Basak}, R. and {Tam}, P.~H.~T. and {Sharma}, Vidushi and {Pand
        ey}, S.~B. and {Kumar}, Amit and {Yang}, Yi-Si},
        title = "{Peculiar prompt emission and afterglow in H.E.S.S. detected GRB 190829A}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - High Energy Astrophysical Phenomena},
         year = 2020,
        month = jan,
          eid = {arXiv:2001.00648},
        pages = {arXiv:2001.00648},
archivePrefix = {arXiv},
       eprint = {2001.00648},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020arXiv200100648C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@MISC{2019sptz.prop14317L,
       author = {{Levan}, Andrew and {Tanvir}, Nial and {Fruchter}, Andrew and
         {Lamb}, Gavin and {Hjorth}, Jens and {Malesani}, Daniele and
         {Heintz}, Kasper and {Perley}, Daniel and {Fynbo}, Johan and
         {Wiersema}, Klaas and {Bolmer}, Jan and {Pian}, Elena and
         {Schulze}, Steve and {Izzo}, Luca},
        title = "{Do collapsars create the heaviest elements?}",
 howpublished = {Spitzer Proposal},
         year = 2019,
        month = sep,
        pages = {14317},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019sptz.prop14317L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2019GCN.25682....1V,
       author = {{Volnova}, A. and {Rumyantsev}, V. and {Pozanenko}, A. and {Belkin}, S. and
         {Mazaeva}, E. and {IKI GRB FuN Collaboration}},
        title = "{GRB 190829A observations in CrAO, photometry of the SN}",
      journal = {GRB Coordinates Network},
         year = 2019,
        month = sep,
       volume = {25682},
        pages = {1},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019GCN.25682....1V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2019GCN.25677....1D,
       author = {{de Ugarte Postigo}, A. and {Izzo}, L. and {Thoene}, C.~C. and
         {Blazek}, M. and {Bensch}, K. and {Agui}, J.~F. and {Kann}, D.~A. and
         {Cabrera Lavers}, A.~L. and {Castro-Rodriguez}, N. and
         {Tejero Caro}, A.},
        title = "{GRB 190829A: GTC confirmation of an associated Type Ic-BL Supernova}",
      journal = {GRB Coordinates Network},
         year = 2019,
        month = sep,
       volume = {25677},
        pages = {1},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019GCN.25677....1D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2019GCN.25676....1L,
       author = {{Laskar}, T. and {Bhandari}, S. and {Schroeder}, G. and {Fong}, W. and
         {Alexander}, K.~D. and {Berger}, E. and {Chornock}, R. and
         {Coppejans}, D. and {Margutti}, R. and {Ayache}, E. and
         {Mundell}, C.~G. and {Schady}, P. and {van Eerten}, H.~J. and {et al.}},
        title = "{GRB 190829A: ATCA cm-band detection}",
      journal = {GRB Coordinates Network},
         year = 2019,
        month = sep,
       volume = {25676},
        pages = {1},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019GCN.25676....1L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2019GCN.25667....1V,
       author = {{Vagnozzi}, A. and {Nesci}, R.},
        title = "{GRB 190829A optical observation}",
      journal = {GRB Coordinates Network},
         year = 2019,
        month = sep,
       volume = {25667},
        pages = {1},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019GCN.25667....1V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2019GCN.25664....1T,
       author = {{Terreran}, G. and {Fong}, W. and {Margutti}, R. and {Miller}, A. and
         {Alexander}, K. and {Blanchard}, P. and {Coppejans}, D. and
         {Paterson}, K.},
        title = "{GRB190829A: Keck LRIS spectroscopic confirmation of the accompanying supernova}",
      journal = {GRB Coordinates Network},
         year = 2019,
        month = sep,
       volume = {25664},
        pages = {1},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019GCN.25664....1T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2019GCN.25660....1T,
       author = {{Tsvetkova}, A. and {Golenetskii}, S. and {Aptekar}, R. and
         {Frederiks}, D. and {Ulanov}, M. and {Svinkin}, D. and {Lysenko}, A. and
         {Kozlova}, A. and {Cline}, T. and {Konus-Wind Team}},
        title = "{Konus-Wind observation of GRB 190829A}",
      journal = {GRB Coordinates Network},
         year = 2019,
        month = sep,
       volume = {25660},
        pages = {1},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019GCN.25660....1T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2019GCN.25657....1P,
       author = {{Perley}, D.~A. and {Cockeram}, A.~M.},
        title = "{GRB 190829A: Liverpool Telescope observations of a slow supernova rise}",
      journal = {GRB Coordinates Network},
         year = 2019,
        month = sep,
       volume = {25657},
        pages = {1},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019GCN.25657....1P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2019GCN.25652....1L,
       author = {{Lipunov}, V. and {Balakin}, F. and {Gorbovskoy}, E. and {Kornilov}, V. and
         {Tyurina}, N. and {Balanutsa}, P. and {Kuznetsov}, A. and
         {Vladimirov}, V. and {Vlasenko}, D. and {Gorbunov}, I. and
         {Zimnukhov}, D. and {Senik}, V. and {Pogrosheva}, T. and
         {Kuvshinov}, D. and {Podesta}, R. and {Lopez}, C. and {Podesta}, F. and
         {Francile}, C. and {Levato}, H. and {Rebolo}, R. and {Serra}, M. and
         {Buckley}, D. and {Gres}, O.~A. and {Budnev}, N.~M. and {Ershova}, O. and
         {Tlatov}, A. and {Dormidontov}, D. and {Yurkov}, V. and {Gabovich}, A. and
         {Sergienko}, Yu.},
        title = "{GRB 190829A: MASTER confirmation of GROND SN}",
      journal = {GRB Coordinates Network},
         year = 2019,
        month = sep,
       volume = {25652},
        pages = {1},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019GCN.25652....1L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2019GCN.25651....1B,
       author = {{Bolmer}, J. and {Greiner}, J. and {Chen}, T. -W.},
        title = "{GRB190829A: GROND detection of the accompanying SN}",
      journal = {GRB Coordinates Network},
         year = 2019,
        month = sep,
       volume = {25651},
        pages = {1},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019GCN.25651....1B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2019GCN.25641....1S,
       author = {{Strausbaugh}, R. and {Cucchiara}, A. and {et al.}},
        title = "{GRB 190829A: LCO Optical Afterglow Detection}",
      journal = {GRB Coordinates Network},
         year = 2019,
        month = sep,
       volume = {25641},
        pages = {1},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019GCN.25641....1S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2019GCN.25635....1M,
       author = {{Monageng}, I. and {van der Horst}, A.~J. and {Woudt}, P.~A. and
         {Bottcher}, M. and {et al.}},
        title = "{GRB 190829A: MeerKAT radio observation}",
      journal = {GRB Coordinates Network},
         year = 2019,
        month = sep,
       volume = {25635},
        pages = {1},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019GCN.25635....1M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2019GCN.25627....1C,
       author = {{Chandra}, Poonam and {et al.}},
        title = "{GRB 190829A: Detection of radio afterglow with the uGMRT}",
      journal = {GRB Coordinates Network},
         year = 2019,
        month = sep,
       volume = {25627},
        pages = {1},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019GCN.25627....1C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2019GCN.25623....1P,
       author = {{Perley}, D.~A. and {Cockeram}, A.~M.},
        title = "{GRB 190829A: Flattening of optical light curve from continued Liverpool Telescope photometry}",
      journal = {GRB Coordinates Network},
         year = 2019,
        month = sep,
       volume = {25623},
        pages = {1},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019GCN.25623....1P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2019GCN.25597....1P,
       author = {{Perley}, D.~A. and {Cockeram}, A.~M.},
        title = "{GRB 190829A: Continued fading inferred from Liverpool Telescope photometry}",
      journal = {GRB Coordinates Network},
         year = 2019,
        month = sep,
       volume = {25597},
        pages = {1},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019GCN.25597....1P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2019GCN.25595....1D,
       author = {{de}, K. and {Karambelkar}, V. and {Kasliwal}, M.~M. and
         {Growth Collaboration}},
        title = "{GRB 190829A: Keck LRIS spectroscopy of the optical afterglow}",
      journal = {GRB Coordinates Network},
         year = 2019,
        month = aug,
       volume = {25595},
        pages = {1},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019GCN.25595....1D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2019GCN.25592....1B,
       author = {{Blazek}, M. and {Kann}, L. Izzo. D.~A. and {de Ugarte-Postigo}, A. and
         {Thoene}, C.~C.},
        title = "{GRB 190829A: Liverpool Telescope observations}",
      journal = {GRB Coordinates Network},
         year = 2019,
        month = aug,
       volume = {25592},
        pages = {1},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019GCN.25592....1B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2019GCN.25591....1D,
       author = {{D'Avanzo}, P. and {D'Elia}, V. and {Rossi}, A. and {Melandri}, A. and
         {De Pasquale}, M. and {Malesani}, D.~B. and {Andreuzzi}, G. and
         {Garcia de Gurtubai Escudero}, A. and {Carleo}, I. and
         {CIBO Collaboration}},
        title = "{GRB 190829A: TNG imaging of the NIR afterglow}",
      journal = {GRB Coordinates Network},
         year = 2019,
        month = aug,
       volume = {25591},
        pages = {1},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019GCN.25591....1D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2019GCN.25589....1D,
       author = {{de Ugarte Postigo}, A. and {Bremer}, M. and {Kann}, D.~A. and
         {Schulze}, S. and {Thoene}, C.~C. and {Blazek}, M. and {Bensch}, K. and
         {Agui}, J.~F. and {Izzo}, L. and {Perley}, D.~A. and {Martin}, S. and
         {de Gregorio-Monsalvo}, I. and {Michalowski}, M. and {Malesani}, D.~B. and
         {Sanchez-Ramirez}, R.},
        title = "{GRB 190829A: NOEMA detection of the mm afterglow}",
      journal = {GRB Coordinates Network},
         year = 2019,
        month = aug,
       volume = {25589},
        pages = {1},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019GCN.25589....1D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2019GCN.25585....1P,
       author = {{Perley}, D.~A. and {Cockeram}, A.~M.},
        title = "{GRB 190829A: Liverpool Telescope optical photometry}",
      journal = {GRB Coordinates Network},
         year = 2019,
        month = aug,
       volume = {25585},
        pages = {1},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019GCN.25585....1P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2019GCN.25584....1P,
       author = {{Paek}, Gregory S.~H. and {Im}, Myungshin and {et al.}},
        title = "{GRB 190829A: UKIRT detection of the NIR Afterglow}",
      journal = {GRB Coordinates Network},
         year = 2019,
        month = aug,
       volume = {25584},
        pages = {1},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019GCN.25584....1P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2019GCN.25583....1F,
       author = {{Fong}, W. and {Laskar}, T. and {Schroeder}, G. and {Coppejans}, D. and
         {Margutti}, R.},
        title = "{GRB 190829A: MMT detection of the optical afterglow}",
      journal = {GRB Coordinates Network},
         year = 2019,
        month = aug,
       volume = {25583},
        pages = {1},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019GCN.25583....1F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2019GCN.25582....1C,
       author = {{Coleiro}, Alexis and {Dornic}, Damien and {ANTARES Collaboration}},
        title = "{GRB 190829A: No Neutrino Counterpart detected with ANTARES}",
      journal = {GRB Coordinates Network},
         year = 2019,
        month = aug,
       volume = {25582},
        pages = {1},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019GCN.25582....1C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2019GCN.25581....1D,
       author = {{Dado}, S. and {Dar}, A.},
        title = "{GRB 190829A: Follow up VLA and VLBI radio observations urged}",
      journal = {GRB Coordinates Network},
         year = 2019,
        month = aug,
       volume = {25581},
        pages = {1},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019GCN.25581....1D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2019GCN.25580....1Z,
       author = {{Zheng}, WeiKang and {Filippenko}, Alexei V. and {KAIT GRB Team}},
        title = "{GRB 190829A: KAIT Detection of the Optical Afterglow}",
      journal = {GRB Coordinates Network},
         year = 2019,
        month = aug,
       volume = {25580},
        pages = {1},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019GCN.25580....1Z},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2019GCN.25579....1L,
       author = {{Lien}, A.~Y. and {Barthelmy}, S.~D. and {Cummings}, J.~R. and
         {Dichiara}, S. and {Krimm}, H.~A. and {Markwardt}, C.~B. and
         {Palmer}, D.~M. and {Sakamoto}, T. and {Stamatikos}, M. and
         {Ukwatta}, T.~N. and {Swift-BAT Team}},
        title = "{GRB 190829A, Swift-BAT refined analysis}",
      journal = {GRB Coordinates Network},
         year = 2019,
        month = aug,
       volume = {25579},
        pages = {1},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019GCN.25579....1L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2019GCN.25578....1P,
       author = {{Piano}, G. and {Verrecchia}, F. and {Tavani}, M. and {Pittori}, C. and
         {Ursi}, A. and {Cardillo}, M. and {Casentini}, C. and {Lucarelli}, F. and
         {Bulgarelli}, A. and {Fioretti}, V. and {Parmiggiani}, N. and
         {Pilia}, M. and {Longo}, F. and {Agile Team}},
        title = "{GRB 190829A: AGILE-GRID upper limits}",
      journal = {GRB Coordinates Network},
         year = 2019,
        month = aug,
       volume = {25578},
        pages = {1},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019GCN.25578....1P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2019GCN.25577....1P,
       author = {{Pittori}, C. and {Ursi}, A. and {Tavani}, M. and {Cardillo}, M. and
         {Casentini}, C. and {Piano}, G. and {Lucarelli}, F. and
         {Verrecchia}, F. and {Bulgarelli}, A. and {Fioretti}, V. and
         {Parmiggiani}, N. and {Pilia}, M. and {Longo}, F. and {Agile Team}},
        title = "{GRB 190829A: AGILE ratemeters detection and MCAL upper limits}",
      journal = {GRB Coordinates Network},
         year = 2019,
        month = aug,
       volume = {25577},
        pages = {1},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019GCN.25577....1P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2019GCN.25575....1L,
       author = {{Lesage}, S. and {Poolakkil}, S. and {Fletcher}, C. and {Meegan}, C. and
         {Goldstein}, A. and {Fermi GBM Team}},
        title = "{GRB 190829A: Fermi GBM detection}",
      journal = {GRB Coordinates Network},
         year = 2019,
        month = aug,
       volume = {25575},
        pages = {1},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019GCN.25575....1L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2019GCN.25574....1P,
       author = {{Piron}, F. and {Longo}, F. and {Axelsson}, M. and {Arimoto}, M. and
         {Racusin}, J.~L. and {Bissaldi}, E. and {Fermi-LAT Collaboration}},
        title = "{GRB 190829A: Fermi-LAT Upper Limits}",
      journal = {GRB Coordinates Network},
         year = 2019,
        month = aug,
       volume = {25574},
        pages = {1},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019GCN.25574....1P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2019GCN.25573....1L,
       author = {{Lipunov}, V. and {Gorbovskoy}, E. and {Balakin}, F. and {Kornilov}, V. and
         {Tyurina}, N. and {Balanutsa}, P. and {Kuznetsov}, A. and
         {Vladimirov}, V. and {Vlasenko}, D. and {Gorbunov}, I. and
         {Zimnukhov}, D. and {Senik}, V. and {Pogrosheva}, T. and
         {Kuvshinov}, D. and {Chasovnikov}, A. and {Topolev}, V. and
         {Posdnyakov}, A. and {Yurkov}, V. and {Gabovich}, A. and
         {Sergienko}, Yu. and {Tlatov}, A. and {Dormidontov}, D. and
         {Podesta}, R. and {Lopez}, C. and {Podesta}, F. and {Francile}, C. and
         {Levato}, H. and {Rebolo}, R. and {Serra}, M. and {Buckley}, D. and
         {Gres}, O.~A. and {Budnev}, N.~M. and {Ershova}, O.},
        title = "{GRB 190829A:: Global MASTER-net optical clear and polarization observations scheduler and some spiculations}",
      journal = {GRB Coordinates Network},
         year = 2019,
        month = aug,
       volume = {25573},
        pages = {1},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019GCN.25573....1L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2019GCN.25570....1O,
       author = {{Oates}, S.~R. and {Dichiara}, S. and {Swift/UVOT Team}},
        title = "{GRB 190829A: Swift/UVOT detection of an optical afterglow with a rise}",
      journal = {GRB Coordinates Network},
         year = 2019,
        month = aug,
       volume = {25570},
        pages = {1},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019GCN.25570....1O},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2019GCN.25569....1C,
       author = {{Chen}, T. -W. and {Bolmer}, J. and {Nicuesa Guelbenzu}, A. and
         {Klose}, S.},
        title = "{GRB 190829A: GROND detection of the Optical/NIR Afterglow}",
      journal = {GRB Coordinates Network},
         year = 2019,
        month = aug,
       volume = {25569},
        pages = {1},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019GCN.25569....1C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2019GCN.25568....1O,
       author = {{Osborne}, J.~P. and {Page}, K.~L. and {Capalbi}, M. and {Perri}, M. and
         {D'Elia}, V. and {Burrows}, D.~N. and {Gropp}, J.~D. and
         {Tohuvavohu}, A. and {Beardmore}, A.~P. and {Dichiara}, S. and
         {Swift-XRT Team}},
        title = "{GRB 190829A: Swift-XRT refined Analysis}",
      journal = {GRB Coordinates Network},
         year = 2019,
        month = aug,
       volume = {25568},
        pages = {1},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019GCN.25568....1O},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2019GCN.25567....1E,
       author = {{Evans}, P.~A. and {Goad}, M.~R. and {Osborne}, J.~P. and
         {Beardmore}, A.~P. and {Swift-XRT Team}},
        title = "{GRB 190829A: Enhanced Swift-XRT position}",
      journal = {GRB Coordinates Network},
         year = 2019,
        month = aug,
       volume = {25567},
        pages = {1},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019GCN.25567....1E},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2019GCN.25566....1D,
       author = {{de Naurois}, M. and {H.~E.~S.~S. Collaboration}},
        title = "{GRB190829A: Detection of VHE gamma-ray emission with H.E.S.S.}",
      journal = {GRB Coordinates Network},
         year = 2019,
        month = aug,
       volume = {25566},
        pages = {1},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019GCN.25566....1D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2019GCN.25565....1V,
       author = {{Valeev}, A.~F. and {Castro-Tirado}, A.~J. and {Hu}, Y. -D. and {Fernand
        ez-Garcia}, E. and {Sokolov}, V.~V. and {Carrasco}, I. and
         {Castellon}, A. and {Garcia Alvarez}, D. and {Rivero}, M. and {et al.}},
        title = "{GRB 190829A: 10.4m GTC spectroscopy}",
      journal = {GRB Coordinates Network},
         year = 2019,
        month = aug,
       volume = {25565},
        pages = {1},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019GCN.25565....1V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2019GCN.25563....1H,
       author = {{Heintz}, K.~E. and {Fynbo}, J.~P.~U. and {Jakobsson}, P. and {Xu}, D. and
         {Perley}, D.~A. and {Malesani}, D.~B. and {Viuho}, J. and {et al.}},
        title = "{GRB 190829A: NOT optical afterglow detection and spectroscopy}",
      journal = {GRB Coordinates Network},
         year = 2019,
        month = aug,
       volume = {25563},
        pages = {1},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019GCN.25563....1H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2019GCN.25560....1K,
       author = {{Kumar}, H. and {Bhalerao}, V. and {Stanzin}, Jigmat and
         {Anupama}, G.~C. and {Barwe}, S. and {Growth-India Collaboration}},
        title = "{GRB 190829A: GROWTH India detection of afterglow}",
      journal = {GRB Coordinates Network},
         year = 2019,
        month = aug,
       volume = {25560},
        pages = {1},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019GCN.25560....1K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2019GCN.25558....1L,
       author = {{Lipunov}, V. and {Balakin}, F. and {Gorbovskoy}, E. and {Kornilov}, V. and
         {Tyurina}, N. and {Balanutsa}, P. and {Kuznetsov}, A. and
         {Vladimirov}, V. and {Vlasenko}, D. and {Gorbunov}, I. and
         {Zimnukhov}, D. and {Senik}, V. and {Pogrosheva}, T. and
         {Kuvshinov}, D. and {Podesta}, R. and {Lopez}, C. and {Podesta}, F. and
         {Francile}, C. and {Levato}, H. and {Rebolo}, R. and {Serra}, M. and
         {Gres}, O.~A. and {Budnev}, N.~M. and {Ershova}, O. and {Tlatov}, A. and
         {Dormidontov}, D. and {Yurkov}, V. and {Gabovich}, A. and
         {Sergienko}, Yu.},
        title = "{GRB 190829A:: MASTER-net bright and decay OT detection}",
      journal = {GRB Coordinates Network},
         year = 2019,
        month = aug,
       volume = {25558},
        pages = {1},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019GCN.25558....1L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2019GCN.25555....1X,
       author = {{Xu}, D. and {Yu}, B.~Y. and {Zhu}, Z.~P. and {et al.}},
        title = "{GRB 190829A: Dabancheng-0.5m optical afterglow detection}",
      journal = {GRB Coordinates Network},
         year = 2019,
        month = aug,
       volume = {25555},
        pages = {1},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019GCN.25555....1X},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2019GCN.25552....1D,
       author = {{Dichiara}, S. and {Bernardini}, M.~G. and {Burrows}, D.~N. and
         {D'Avanzo}, P. and {Gronwall}, C. and {Gropp}, J.~D. and
         {Kennea}, J.~A. and {Klingler}, N.~J. and {Krimm}, H.~A. and
         {Kuin}, N.~P.~M. and {LaPorte}, S.~J. and {Melandri}, A. and
         {Page}, K.~L. and {Palmer}, D.~M. and {Siegel}, M.~H. and
         {Simpson}, K.~K. and {Tohuvavohu}, A. and
         {Neil Gehrels Swift Observatory Team}},
        title = "{GRB 190829A: Swift detection of a burst consistent with a galaxy at z=0.08}",
      journal = {GRB Coordinates Network},
         year = 2019,
        month = aug,
       volume = {25552},
        pages = {1},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019GCN.25552....1D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2019GCN.25551....1F,
       author = {{Fermi GBM Team}},
        title = "{GRB 190829A: Fermi GBM Final Real-time Localization}",
      journal = {GRB Coordinates Network},
         year = 2019,
        month = aug,
       volume = {25551},
        pages = {1},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019GCN.25551....1F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2019ATel13057....1C,
       author = {{Coleiro}, Alexis and {Dornic}, Damien},
        title = "{GRB 190829A: No Neutrino Counterpart detected with ANTARES}",
      journal = {The Astronomer's Telegram},
     keywords = {Gamma-Ray Burst},
         year = 2019,
        month = aug,
       volume = {13057},
        pages = {1},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019ATel13057....1C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2019ATel13052....1D,
       author = {{de Naurois}, M.},
        title = "{GRB190829A: Detection of VHE gamma-ray emission with H.E.S.S.}",
      journal = {The Astronomer's Telegram},
     keywords = {Gamma-Ray Burst},
         year = 2019,
        month = aug,
       volume = {13052},
        pages = {1},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019ATel13052....1D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


